Understanding Content Placement Strategies in Smartrouter-based Peer CDN for Video Streaming

Recent years have witnessed a new video delivery paradigm: smartrouter-based peer video content delivery network, which is enabled by smartrouters deployed at users' homes. ChinaCache (one of the largest CDN providers in China) and Youku (a video provider using smartrouters to assist video delivery) announced their cooperation in 2015, to create a new paradigm of content delivery based on householders' network resources. This new paradigm is different from the conventional peer-to-peer (P2P) approach, because millions of dedicated smartrouters are operated by the centralized video service providers in a coordinative manner. Thus it is intriguing to study the content placement strategies used in a smartrouter-based content delivery system, as well as its potential impact on the content delivery ecosystem. In this paper, we carry out measurement studies of Youku's peer video CDN, who has deployed over 300K smartrouter devices for its video delivery. In our measurement studies, 104K videos were investigated and 4TB traffic has been analyzed, over controlled smartrouter nodes and players. Our measurement insights are as follows. First, a global content replication strategy is essential for the peer CDN systems. Second, such peer CDN deployment itself can form an effective sub-system for end-to-end QoS monitoring, which can be used for fine-grained request redirection (e.g., user-level) and content replication. We also show our analysis on the performance limitations and propose potential improvements to the peer CDN systems.

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}

This work is supported in part by the National Natural Science Foundation of China (NSFC) under Grant No.~61133008, 61472204 and 61531006, Beijing Key Laboratory of Networked Multimedia, and the National Basic Research Program of China (973) under Grant No.~2015CB352300.


==> sections/architecture.tex <==
\section{Measurement Methodology}  \label{MeasurementMethodology}

We conduct both active and passive measurement on clients and the peer CDN nodes in our study.
 
 
\begin{figure}[!t]		
	\centering
	\includegraphics[width=0.8\linewidth]{icmeframework.eps}
	\caption{The frame of AP-based peer CDN monitor system.}
	\label{fig:monitorframe}
\end{figure} 	

\subsection{Measurement by Controlled Peer CDN Nodes}

\subsubsection{Testing Node Deployment}

We use $5$ Youku smartrouters in our measurement study, which are deployed in different locations with different ISPs. As illustrated in Fig.~\ref{fig:nodelocation}, the $5$ routers are denoted as follows: 

    \rhd [\textsf{R1},\textsf{R2},] which is deployed in Beijing (ISP: CERNET), with public IP address and $80$ Mbps downlink/uplink bandwidth;  
    
     \rhd [\textsf{R3},] which is deployed in Beijing (ISP: CERNET), with private IP (NAT) and $80$ Mbps downlink/uplink bandwidth;

     \rhd [\textsf{R4},] which is deployed in Beijing (ISP: China Unicom), with public IP and $2$ Mbps downlink bandwidth and $512$ Kbps uplink bandwidth;
    
   \rhd [\textsf{R5},] which is deployed in Shenzhen (ISP: CERNET), with private IP address and $80$ Mbps downlink/uplink bandwidth.

\end{itemize}

\begin{figure}[!t]		
	\centering
	\includegraphics[width=0.8\linewidth]{measurenode.eps}
	\caption{Deployment of testing peer CDN nodes.}
	\label{fig:nodelocation}
\end{figure} 	


\subsubsection{Device Information}

We use the ordinary version of Youku smartrouters as our testing nodes, which have the hardware information as illustrated in Table \ref{tab:smartroutercost}. In particular, the devices provide a MIPS $580$MHz CPU, and the capacity of the storage based on $4$ TF cards is $8$GB.

	
\begin{table}[!t]
  \caption{Hardware information of controlled testing nodes. }
  \label{tab:smartroutercost}
  \centering  
   %\begin{threeparttable}
  \begin{tabular}{ll}%{ *3{>{\centering\arraybackslash}m{1.5 in}} @{}m{0pt}@{}}
    \toprule
        Parameter	&	Information \\
    \midrule
        CPU				&	$580$MHz	\\
        RAM				&	128MB (DDR2)	\\
	    Operating System	&	OpenWrt 2.6.36	\\
	    WiFi Protocol/Channel   & IEEE 802.11 b/g/n@2.4 GHz	\\
	     Storage &  8GB (4 $\times$ TF cards 	\\
         Price		&	26.3USD (December 2015)	\\    
     \bottomrule
  \end{tabular}
\end{table}

Next, we present our measurement on these devices. 


\subsubsection{File System Monitoring}

In our experiments, we degrade the version of the OpenWrt OS 2.6 on these devices, such that we are able to connect these devices via SSH. We monitor the folders on the devices where \emph{video files} are stored to serve users. In Youku peer CDN, all contents are cached as video chunks with an unique content ID, and our experiments cover $78$K different videos during the monitoring period. In Sec.~\ref{section:chunk}, we will present the details of the file monitoring results. 


\subsubsection{Traffic Monitoring}

We also monitor the traffic patterns on these devices, using the conventional network utility tools including \textsf{tcpdump}, \textsf{netstat}, etc. Table \ref{tab:datasets} illustrates a statistics in our measurement experiments. In particular, our experiments last for over $40$ days, and over $78$k videos are monitored in the file systems.

\begin{table}[!t]
  \caption{Statistics in our measurement studies.}
  \label{tab:datasets}
  \centering  
    \begin{tabular}{p{.65\linewidth}p{.35\linewidth}}
    \toprule
     Time period		&	Sept 15  -- Oct 31, 2015	\\
    \midrule 
     Video number	    & 78,285 \\
     TCP Packets				&	4,438,510,988	\\
	 Contacted servers	    &	126		\\
	 Contacted IPs				&  	3,155,877\\
	 Distinct ASes			&  4,015\\
    \bottomrule
  \end{tabular}
\end{table}
 

\subsection{Measurement by Controlled Clients}

In our study, we also run testing clients to join the system and measure their interactions with the peer CDN nodes (including both our testing nodes and others). We act as ordinary users who request a number of videos, and monitor how these requests are served by the system.





==> sections/discussion.tex <==
\section{Discussion} \label{sec:discussion} TODO: 删除本节

In this section, we discuss the limitation of our measurement and propose two potential principles which can be influential for the peer CDN design.

TODO: 下面移到移动到去一部分

$\rhd$ Limitation: 1) According to the results, the behaviors of our 5 peer routers demonstrate certain consistent patterns. However, it is still possible that some scenarios are not captured by our deployed peer routers. 2) In order to effectively serve users, massive amount of videos are continuously replicated between peer routers, which consumes too much user-side bandwidth. In our measurement, distinguishing that contents are uploaded to users or other peer routers is difficult due to all of the connection establishing based on the same P2P protocols. But it is worthy to compare the edge-network bandwidth consumption with the CDN peak-traffic offloading.

TODO: 下面移到移动到conclusion最后

$\rhd$ Potential improvement: 1) \textbf{Global QoS monitoring based on Peer routers}. Through the traffic datasets analysis, we observe that a large amount of flows between peer routers maintain long time but light load connections. We speculate that there are probing flows for making peer routers keep contact with their partners. Since the CDN control plane can obtain the end-to-end QoS information from the large scale peer router swarm, it would be influential for the entire network perception and fine-grained user request redirection. 
%2) \textbf{Regional content replication}. In our experiment, videos are replicated in a global coordinative manner, but the content popularity of different regions is diverse\footnote{https://www.youtube.com/trendsmap}. If we want peer routers to provide a efficient nearby service, balancing the regional content popularity and global content popularity is important for the replication strategy design in peer CDN. 
2) \textbf{fine-grained content placement}. Due to the significant storage space and the low cost for the content placement in peer CDN, control plane can efficiently schedule the copy number for any video. This feature should be fully utilized to meet many sophisticated demands for system optimization, such as a more accurate popularity prediction algorithm and a newly official recommendation on the frontpage.

%Based on our analysis, compared to the conventional CDN which manages the QoS between edge servers and end users and updates the contents for a large region, tapping the internal potential of peer CDN is promising to provide more efficient video service.


%In Fig.~\ref{fig:linknum}. we estimate the number of peers traced for each chunk in \textsf{R1}, by counting the number connection issued by our peer router during a chunk downing period, and we observe that for one chunk downloading, the average number of traced peers are up to $250$.
 

 
% \begin{figure}[t] 
%
%  \begin{subfigure}[t]{0.47\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{avg_byte_connection.eps} 
%   \caption{The CDF of average packet load per connection.}
%  \end{subfigure} 
%  \hfill
%    \begin{subfigure}[t]{0.47\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{stream_cdf_tracenumber} 
%    \caption{The number of peers traced for each chunk.}  
%  \end{subfigure}%% 
% % \hfill
%     \caption{Monitoring traffic in \textsf{R1}.}  
%
%  \label{fig:linknum}
%  		 
%\end{figure}



==> sections/incentive.tex <==

\subsection{Incentive Mechanism} \label{section:incentive}
%Third, inventive mechanisms are critical for peer CDN systems, and dynamical incentive strategies are in demand to improve the QoS for users.


Content providers resort to peer CDN to reduce their bandwidth rental cost from the datacenters, which is still one of the main budget nowadays, i.e., in the China Cycomm datacenters, the bandwidth price is \$25/month/M.
	
	Traditional P2P system generally designs tit-for-tat and simple strategies to urge their peers upload the local content resources, such as they would punish slow uploaders \cite{cohen2003incentives}. Whereas in the peer CDN system, more inventive mechanisms are in demand to stimulate their users to contribute their upload bandwidth for the content distribution. Because users can always obtain the content from the CDN edge servers, even if they never produce fruit \cite{Akamai}. 

	In this section, we introduce and analysis the inventive mechanisms adopted by Youku to encourage the peer router owners allowing the their smartrouter to share the upload capacities. 

\textbf{Virtual Coin}: Youku pays the Youku Virtual Coins, which can be converted into actual money or some discount coupon of Youku partners, to the owner of the Youku router who contribute their upload bandwidth. It is the main reward strategy to arouse the user intentions. Each Youku account can bind with multiple Youku routers and manage the virtual coins.

 Due to the calculation formula of virtual coin is not available in the Youku website, we study the concrete relationship between the amount of upload traffic and the number of virtual coins earned in Fig.~\ref{fig:coin}. We plot the virtual coin earned during the monitoring period of our 4 routers, and each sample represents information of one day (the virtual coins was given by day). We can find a simple linear relationship between the upload traffic and the virtual coins, whose slope is 8.3 coin/GB. 
 
 By the end of the Oct 31 st, 2015, we earned 13161 virtual coins in total from our 4 peer routers. We list some of the typical commodities to which virtual coins can convert. If we directly acquire the cash, we only get \$3.6; but if we are the client of DaoWei APP, we would enjoy the service which values \$1021. This agile rewarding strategy can successful interest the owners of Youku peer routers to contribute their surplus bandwidth, while Youku pays them at a very low cost, only 8.3 virtual coins per GB (\$0.002/GB).
 
 
 \begin{table}[!htbp]
  \caption{The value of virtual coin.}
  \label{tab:coin_value}
  \centering  
   %\begin{threeparttable}
  \begin{tabular}{ccc}%{ *3{>{\centering\arraybackslash}m{1.5 in}} @{}m{0pt}@{}}
    \toprule
    Exchangeable commodity	& Virtual coins		&   		Value	 \\
    \midrule
    Cash					& 8000					     		& 		\$2.16\\
    One month VIP subscriber 	 & 6400							& 		\$2.16\\
    One month AD filter	&	4800										&		\$1.86 \\
	Coupons from DaoWei APP 		& 100							&	\$7.81	\\
	%	... 		& ...							&	...\\
       \bottomrule
  \end{tabular}
\end{table}
 
\textbf{Incentive-aware content placement}: 	
	 \begin{figure*}[t] 
	 \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk2ip.eps} 
    \caption{The number of chunks downloaded by each peer during one day.}  
  \end{subfigure}%% 
  \hfill
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_views1.eps} 
    \caption{The CDF of the number of daily views at the same day for the chunks of the router \textsf{R1}.}  
  \end{subfigure}%% 
  \hfill
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_alldays.eps} 
   \caption{The CDF of the number of total views for the chunks of the router \textsf{R1}.}
  \end{subfigure}  
      \caption{The incentive-aware content placement strategy.}
 		 \label{fig:chunkincentive}
\end{figure*}
 \begin{figure*}[!t]
\begin{minipage}[t]{0.31\linewidth} %0.215

    \centering
    \includegraphics [width=\linewidth, height=3.6cm]{chunk_views1_pl.eps}
    \centerline{\scriptsize (a) Video daily popularity .}
  \end{minipage}
  \hfill
\begin{minipage}[t]{0.28\linewidth} %0.215
    \centering
    \includegraphics [width=1\linewidth, height=4cm]{chunk_alldays_pl.eps}
		\centerline{\scriptsize (b) Video total popularity.}
  \end{minipage}
  \hfill

 \caption{The characteristics of chunk replication scheduling.}
  \label{fig:chunkscheduling}
   \vspace{-0.4cm}
 \end{figure*}
 
With incentive-aware content placement strategy analysed above, Youku build a completely new smartrouter-based peer CDN ecosystem and produce a win-win and fair situation for all of the end-users.

==> sections/monitor.tex <==

%Further, we investigate the degree of parallel downloading adopt by the Youku peer router. As for downloading chuck with different size, the concurrent connections is all different. 
%In Fig.~\ref{fig:linknum}(b), we set different threshold to the total amount of data of each connection, to decide whether a connection is transferring chunks, and observe that there will about $17$ concurrent connections to download a chunks when we set the threshold of 200 KB.


==> sections/qos.tex <==
\section{Performance perceived by users} \label{section:qos}
\begin{figure*}[t]
     \begin{minipage}[t]{0.285\linewidth}
          \centering
               \includegraphics[width=\linewidth]{client_demo.eps}
	      \caption{The traffic pattern of a video session in peer CDN.}
	      \label{fig:client_demo}
		% \vspace{-0.6cm}
     \end{minipage}
	\hfill
     \begin{minipage}[t]{0.63\linewidth}
		 			\begin{minipage}[t]{0.49\linewidth}
			  \centering
				   \includegraphics[width=\linewidth, height=3.9cm]{client_cernetbw_inall.eps}
			  \centerline{\scriptsize (a) Edge-server vs. peer CDN Download speed.}
		 \end{minipage}
		 \hfill
		 \begin{minipage}[t]{0.49\linewidth}
			  \centering
				   \includegraphics[width=\linewidth, height=4cm]{client_p2pratio4g.eps}
			 \centerline{\scriptsize (b) Peer CDN efficiency.}
		 \end{minipage}
		 \hfill
		    \caption{The video delivery QoS of peer CDN.}
     \label{fig:client_qos}
  %   client_p2pratio4g.eps
     % \vspace{-0.6cm}
   	\end{minipage} 
   	\hfill
   	    % 	\vspace{-0.6cm}
\end{figure*}


As we know, the QoS performance of conventional P2P tends to be unmanageable and unpredictable. In this section, we study the performance perceived by original users in the video peer CDN. 

Fig.~\ref{fig:client_demo} illustrates the general traffics pattern of a video session. At the beginning, the user starts to download the first part of the chunks from the edge servers; At the same time, she queries the scheduling server for a peer list generated based on the user' location and ISP information. If suitable peers are detected, the user and the selected peer routers attempt to establish connection with each other and delivery chunks. Meanwhile, the downloading from the edge servers continues in parallel; if selected peers are slow or unreliable, the CDN edge server can cover the difference. Then the user experience does not suffer from this instability. We can see this mechanism can overcome the start-up delays in peer CDN and assure the reliability of the video delivery.

 We evaluate the video delivery performance in Beijing with different network environment, including CERNAT (80 Mbps), Unicom ADSL (2 Mbps), and Unicom 4G (8 Mbps). We choose 450 videos with different popularity based on the most recently played indexes given by Youku website\footnote{\url{ http://index.youku.com/vr_keyword/id_http://v.youku.com/v_show/id_XMjY1MzQwOTQ0.html}}, which follows Zipf distribution, and record the download speed and data ratio come from peers. Fig.~\ref{fig:client_qos}(a) compares the chunk download speed of 1) peer routers transport bytes which larger than 60\% of the chunk, and 2) all bytes are downloaded from CDN edge servers. We can observe the peer CDN has stable download speed in our experiment. Even in th Unicom ADSL and Unicom 4G, peer CDN achieves higher download speed compared to that from edge servers, the reason is that multiple peer routers parallelly accelerate the speed, and there are about up to $15$ concurrent connections to download a chunk in our experiments.
 
 Then we evaluate the peer router delivery ratio and analyze which types of videos can be delivery by peers. Fig.~\ref{fig:client_qos}(b) shows the data ratio delivered by peer routers in our datasets. We observe $80\%$ of the content requests can be served by peer CDN with at least 70\% of the bytes came from peer routers. Most of the videos with lower peer delivering ratio are user generated content (UGC) which are out-of-date. It is worth noting that the out-of-date UGC ``Gangnam Style", which was the most popular videos in many video websites, can keep up with $66\%$ data ratio from peers.
  
  We can calculate as follows: if one drama programme has 20 episodes with the bitrate $1200$Kbps, and each of them have 10000 copies, then $300$K Youku peer routers can cache $4$K different drama programmes, which can meet the interests of most users. It demonstrates network resources of end-user have great potential to provide great video-on-demand service, by utilizing the smartrouter storage and idle uplink bandwidth. 
% The Youku peer CDN serve content to each peer at the best possible speed.
  
 
 \begin{figure*}[t] 
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_httpdays.eps} 
    \caption{The CDF of number of days from the video release to the video downloading to the router \textsf{R1}.}  
  \end{subfigure}%% 
  \hfill
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_httpviews1.eps} 
   \caption{The CDF of the number of daily views for the chunks of the router \textsf{R1}.}
  \end{subfigure}  
  \hfill
    \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_httpalldays.eps} 
    \caption{The CDF of the number of total views for the chunks of the router \textsf{R1}.}  
  \end{subfigure}%% 
  \hfill

      \caption{The comparison between chunks downloaded from Youku servers and peers.}
 		 \label{fig:linknum}
\end{figure*}

 \begin{figure*}[t] 
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_frontdays.eps} 
    \caption{The CDF of number of days from the video release to the video downloaded to the router \textsf{R1}.}  
  \end{subfigure}%% 
  \hfill
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_frontviews1.eps} 
   \caption{The CDF of the number of daily views for the chunks of the router \textsf{R1}.}
  \end{subfigure}  
  \hfill
    \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chunk_frontalldays.eps} 
    \caption{The CDF of the number of total views for the chunks of the router \textsf{R1}.}  
  \end{subfigure}%% 
  \hfill

      \caption{The comparison between chunks on the front webs and Nfront.}
 		 \label{fig:linknum}
\end{figure*}


%
% \begin{figure*}[t] 
%  \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange1.eps} 
%    \caption{TVplay 2015.12.24.}  
%  \end{subfigure}%% 
%  \hfill
%  \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange2.eps} 
%   \caption{.}
%  \end{subfigure}  
%  \hfill
%    \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange3.eps} 
%    \caption{.}  
%  \end{subfigure}%% 
%  \hfill
%  \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange4.eps} 
%    \caption{.}  
%  \end{subfigure}%% 
%  \hfill
%  \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange5.eps} 
%   \caption{.}
%  \end{subfigure}  
%  \hfill
%    \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange6.eps} 
%    \caption{.}  
%  \end{subfigure}%% 
%  \hfill
%    \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange7.eps} 
%    \caption{.}  
%  \end{subfigure}%% 
%  \hfill
%  \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange8.eps} 
%   \caption{.}
%  \end{subfigure}  
%  \hfill
%    \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange9.eps} 
%    \caption{.}  
%  \end{subfigure}%% 
%  \hfill
%      \begin{subfigure}[t]{0.23\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{chunk_seedchange10.eps} 
%    \caption{.}  
%  \end{subfigure}%% 
%  \hfill
%      \caption{Seed changing.}
% 		 \label{fig:linknum}
%\end{figure*}


